Relative Sparsity for Medical Decision Problems

Existing statistical methods can estimate a policy, or a mapping from covariates to decisions, which can then instruct decision makers (e.g., whether to administer hypotension treatment based on covariates blood pressure and heart rate). There is great interest in using such data-driven policies in healthcare. However, it is often important to explain to the healthcare provider, and to the patient, how a new policy differs from the current standard of care. This end is facilitated if one can pinpoint the aspects of the policy (i.e., the parameters for blood pressure and heart rate) that change when moving from the standard of care to the new, suggested policy. To this end, we adapt ideas from Trust Region Policy Optimization (TRPO). In our work, however, unlike in TRPO, the difference between the suggested policy and standard of care is required to be sparse, aiding with interpretability. This yields ``relative sparsity," where, as a function of a tuning parameter, $\lambda$, we can approximately control the number of parameters in our suggested policy that differ from their counterparts in the standard of care (e.g., heart rate only). We propose a criterion for selecting $\lambda$, perform simulations, and illustrate our method with a real, observational healthcare dataset, deriving a policy that is easy to explain in the context of the current standard of care. Our work promotes the adoption of data-driven decision aids, which have great potential to improve health outcomes.

==> table.tex <==
\begin{table}
\tiny
\centering
\begin{tabular}{c|ccccccc}
\hline
             & \thead{Parametric\\ $\pi_{\beta}$} & \thead{Max. \\ value} & \thead{Relative \\sparsity} & \thead{Absolute\\ sparsity} & \thead{Close to\\ behavior} & \thead{Specify\\ behavior} & \thead{Specify value \\or transitions} \\
\hline
Proposed (relative sparsity):\\ $V_n(\beta,b)-\lambda L_1(\beta,b)$ & yes & no & yes & no &  yes & yes &  no \\
\hline
TRPO\cite{schulman2015trust}: \\$V_n(\pi_{\beta},\pi_b)-\lambda KL(\pi_{\beta},\pi_b)$ & no & no & no & no  & yes & yes & no \\
\hline
Absolute relative sparsity: \\$V_n(\beta,b)-\lambda L_0(\beta,b)$ & yes & no & yes & no & no & yes & no \\
%\hline
%Absolute relative sparsity: $V_n(\beta,b) - \lambda L_0(\beta,b)$ & yes & no & no & yes & no & yes & no \\
\hline
Absolute sparsity:\\ $V_n(\beta,b) - \lambda L_0(\beta)$ & yes & no & no & yes & no & yes & no \\
\hline
Absolute sparsity \cite{yang2019regularized}: \\$V_n(\beta,b) - \lambda L_1(\beta)$ & yes & no & no & yes & no & yes & no \\
\hline
Unconstrained\cite{ng2013pegasus}: \\$V_n$ & no & yes & no & no & no  & yes & no \\
\hline
Q-learning\cite{watkins1992q}\\ & no & yes & no & no & no & no  & yes \\
\hline
Sparse Q-learning\cite{song2015penalized}\\ & no & no & no & no & no & no  & yes \\
\hline
Model-based: \\(standard)\cite{sutton2018reinforcement} & no & yes & no & no & no & no & yes \\
\hline
Model-based: \\($V_n-\lambda Likelihood$)\cite{futoma2020popcorn,farahmand2016value} 
& no & yes & no & no & yes & no & yes \\
\hline
\end{tabular}
\caption{ {{\bf The properties of relative sparsity as it relates to other reinforcement learning approaches.} ``Parametric $\pi_{\beta}$'' is whether $\beta$ is parametric. ``Max. value'' indicates whether the policy is optimal with respect to $V_0,$ which will never be the case when there is a penalty.  ``Relative sparsity'' indicates whether there will be only a sparse set of coefficients that differ between the behavioral and suggested policy. ``Absolute sparsity'' indicates whether the policy will have a sparse set of nonzero coefficients, which is equivalent to a relative sparsity to a randomized behavioral policy, which has $b_0=(0,\dots,0)$. ``Close to behavior'' indicates whether the suggested policy probabilities of treatment will be similar to the behavioral policy probabilities of treatment. ``Specify behavior'' indicates whether we must have a model for the behavioral policy; we consider only the policy search ($\arg\max V_n$) objectives for all but the Q-learning and model-based approaches, and hence we consider specification of behavior necessary, because it is necessary for policy search. ``Specify value or transitions'' indicates whether we must propose models for these aspects of the environment and reward structure, which can be non-trivial, and is required in Q-learning and model-based approaches. For the unconstrained approach, we consider the nonparametric optimizer that achieves maximal value. Note that TRPO can be formulated with a parametric policy, $\pi_{\beta}$, but this is not required, and it is often not the case given that the application area is robotics (the policy might be parametric, but it would be over-parameterized as in Deep Learning).}}
\label{qual}
\end{table}
